Certification of projection-based reduced order modelling in computational homogenisation by the Constitutive Relation Error

In this paper, we propose upper and lower error bounding techniques for reduced order modelling applied to the computational homogenisation of random composites. The upper bound relies on the construction of a reduced model for the stress field. Upon ensuring that the reduced stress satisfies the equilibrium in the finite element sense, the desired bounding property is obtained. The lower bound is obtained by defining a hierarchical enriched reduced model for the displacement. We show that the sharpness of both error estimates can be seamlessly controlled by adapting the parameters of the corresponding reduced order model.

==> Homo.tex <==
%!TEX root=POD.tex



==> Presentation.tex <==
%!TEX root=ErrorPOD.tex


\subsection{Elasticity}


\begin{equation}
%\displaystyle 
\forall \, \DispTest \in \SpaceDispZero, \qquad
%\InternalWork (\Stress,\DispTest) + \ExternalWork(\DispTest) = 0 \, ,
\int_\Domain \Stress : \StrainTest \, \DVolume
=
\int_{\Domain} \VolumeForce \cdot \DispTest  \, \DVolume +
\int_{\DDomainNeumann} \NeumannBC \cdot \DispTest   \, \DSurface  \end{equation}

\begin{equation}
\begin{array}{l} 
\displaystyle  \text{Find} \ \Disp(\Parameter) \in \SpaceDisp \ \text{such that}  \ \forall \, \DispTest \in \SpaceDispZero,
\\ \displaystyle  
 a(\Disp(\Parameter),\DispTest ;\Parameter) = l(\DispTest;\Parameter)
\end{array} 
\end{equation}

\begin{equation}
 a(\DispFEM(\Parameter),\DispTest ;\Parameter) = l(\DispTest;\Parameter)
\end{equation}

\subsection{ROM}


\begin{equation}
\DispFEM(\Parameter) 
\approx {\DispReduced}(\Parameter) =  \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter) + \mathbb{P} \, \DirichletBC(\Parameter) 
\end{equation}

\begin{equation} 
 \ErrorReduced^{,\star}(\Parameter) = \DispFEM(\Parameter)   -  \left( \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i}^\star \, \ReducedCoeffI{i}^\star(\Parameter)  + \mathbb{P} \, \DirichletBC(\Parameter) \right)\end{equation}

\begin{equation}
\displaystyle   (\ReducedBasisI{i},\ReducedCoeffI{i})_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } 
= 
\arg
\underset{
(\ReducedBasisI{i}^\star,\ReducedCoeffI{i}^\star)
}{  \text{min} }
\left( \frac{1}{|\ParameterSpace|} \int_\ParameterSpace \left\|  \ErrorReduced^{,\star}(\Parameter) \right\|_{X}^2
\, d\Parameter \right)
\end{equation}

\begin{equation}
\displaystyle   (\ReducedBasisI{i},\ReducedCoeffI{i})_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } 
= \text{arg} \  \min_{(\ReducedBasisI{i}^\star)}
\left( \max_{\ParameterSpace} \left( 
\underset{
 (\ReducedCoeffI{i}^\star)
   }{  \text{min} }
 \left( \left\|  \ErrorReduced^{,\star}(\Parameter) \right\|_{X}^2 \right) \right) \right)
\end{equation} 

\begin{equation}
\begin{array}{ll}
\displaystyle   (\ReducedBasisI{i},\ReducedCoeffI{i})_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } 
& \displaystyle = \arg \underset{
 (\ReducedBasisI{i}^\star,\ReducedCoeffI{i}^\star)
}{  \text{min} }
\left( \frac{1}{|\ParameterSpace|}\int_\ParameterSpace 
a \left(\ErrorReduced^{,\star}(\Parameter), \ErrorReduced^{,\star}(\Parameter); \Parameter \right)
\, d\Parameter \right)
\\ & \displaystyle = 
\underset{
\DispAlt(\Parameter) = \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter) + \mathbb{P} \, \DirichletBC(\Parameter) 
}{  \text{argmin} }
\left(  \frac{1}{|\ParameterSpace|}\int_\ParameterSpace \left( \frac{1}{2}a(\DispAlt(\Parameter),\DispAlt(\Parameter);\Parameter) - l(\DispAlt(\Parameter);\Parameter) \right) \, d\Parameter \right)
\end{array}
\end{equation} 

%\begin{equation}
%\forall \, \DispAlt(\Parameter) = \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter) 
%\end{equation} 


\subsection{POD}


\begin{equation}
\SnapshotZero = \{ \DispFEMHomo(\Parameter)  \Def \DispFEM(\Parameter) - \DispFEMLift(\Parameter) \, | \,  \Parameter \in \ParameterSpaceDiscr \} 
\end{equation}

\begin{equation}
\DispFEM(\Parameter) 
\approx {\DispReduced}(\Parameter) \Def  \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter)  + \DispFEMLift(\Parameter)  
\end{equation}


\begin{equation}
\begin{array}{l}
\displaystyle   (\ReducedBasisI{i})_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } 
= \underset{
( \V{\phi}_i^\star )_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket }  , \, \left<  \V{\phi}_i^\star , \V{\phi}_j^\star \right>_{X}  = \, \delta_{ij} 
}{\text{argmin}} \quad  J \left( ( \V{\phi}_i^\star )_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } \right)
\\ \displaystyle
 J\left( ( \V{\phi}_i^\star )_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } \right)
  = \sum_{\Parameter \in \ParameterSpaceDiscr} \left\| \DispFEMHomo(\Parameter) - \sum_{i=1}^\NumberReducedBasis \left< \DispFEMHomo(\Parameter) , \V{\phi}_i^\star \right>_{X} \ \V{\phi}_i^\star \right\|_{X}
\end{array}
\end{equation}

\begin{equation}
(\ReducedCoeffI{i})_{ i \in \llbracket 1,  \NumberReducedBasis\rrbracket } = \underset{   \Disp^\star(\Parameter) = 
\sum_{i=1}^\NumberReducedBasis \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter)  +  \DispFEMLift(\Parameter)
}{\text{argmin}} \left( \| \DispFEM(\Parameter)  - \Disp^\star(\Parameter)  \|_{\Hooke(\Parameter)} \right)
\end{equation}

\begin{equation}
\StiffnessFEM^\text{r}(\Parameter) \, \ReducedCoeff(\Parameter) = \ForceFEM^\text{r}(\Parameter) + \ForceFEM^\text{r,p}(\Parameter) 
\end{equation}





\begin{equation}
\begin{array}{ll}
\displaystyle
\forall \, \Parameter \in \ParameterSpace, \,  \forall \, \Pos \in \Domain ,  \quad 
& \displaystyle
\Hooke(\Pos,\Parameter) = \sum_{i=1}^\NumberHookeAffine \HookeAffineI{i}(\Pos) \, \CoeffHookeAffineI{i}(\Parameter) 
\\ \displaystyle
\forall \, \Parameter \in \ParameterSpace, \, \forall \, \Pos \in \DDomainNeumann ,  \quad 
& \displaystyle
\NeumannBC(\Pos,\Parameter) = \sum_{i=1}^\NumberNeumannBCAffine \NeumannBCAffineI{i}(\Pos) \, \CoeffNeumannBCAffineI{i}(\Parameter) 
\\ \displaystyle
\forall \, \Parameter \in \ParameterSpace, \, \forall \, \Pos \in \Domain ,  \quad 
& \displaystyle
\VolumeForce(\Pos,\Parameter) = \sum_{i=1}^{\NumberVolumeForceAffine} \VolumeForceAffineI{i}(\Pos) \, \CoeffVolumeForceAffineI{i}(\Parameter) 
\\ \displaystyle
\forall \, \Parameter \in \ParameterSpace, \, \forall \, \Pos \in \DDomainDirichlet , \,  \quad 
& \displaystyle
\DirichletBC(\Pos,\Parameter) = \sum_{i=1}^{\NumberDirichletBCAffine} \DirichletBCAffineI{i}(\Pos) \, \CoeffDirichletBCAffineI{i}(\Parameter) \, ,
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l}
\displaystyle 
%\forall \, \Parameter \in \ParameterSpace, \quad
 \StiffnessFEM^\text{r}(\Parameter) = \sum_{k=1}^\NumberHookeAffine \bar{\StiffnessFEM}^\text{r}_k \, \CoeffHookeAffineI{k}(\Parameter)
\\ \displaystyle \text{where} , \quad 
 \forall \, k \in \llbracket 1 , \NumberHookeAffine \rrbracket , \, \forall \, (i,j) \in \llbracket 1 , \NumberReducedBasis \rrbracket^2 , 
 \,  \quad \quad \bar{\StiffnessFEM}^\text{r}_{k,ij} = 
\bar{a}_k( \ReducedBasisI{j} , \ReducedBasisI{j}) 
\Def \int_\Domain \StrainBasic(\ReducedBasisI{j}) : \HookeAffineI{k}  : \StrainBasic(\ReducedBasisI{i}) \, \DVolume  
\end{array}
\end{equation}




\subsection{Error}

\begin{equation}
\ErrorReduced(\Parameter) \Def \DispFEM(\Parameter) - \DispReduced(\Parameter)
\end{equation}

\begin{equation}
 \CRE(\Parameter) \Def \| \StressReducedHat(\Parameter)  -\Hooke(\Parameter) : \StrainBasic(\DispReduced(\Parameter)) \|_{\Hooke(\Parameter)^{-1}}  \geq \| \ErrorReduced(\Parameter) \|_{\Hooke(\Parameter)}
\end{equation}

\begin{equation}
\forall \, \DispTest \in \SpaceDispFEMZero , \quad
\int_\Domain \StressReducedHat(\Parameter) : \StrainTest \, \DVolume
=
 \int_{\Domain} \VolumeForce(\Parameter) \cdot \DispTest  \, \DVolume +
\int_{\DDomainNeumann} \NeumannBC(\Parameter) \cdot \DispTest   \, \DSurface 
\end{equation}

\begin{equation}
\| \ . \  \|_{\Hooke(\Parameter)} = \left(\int_\Domain \StrainBasic( \ . \ ) : \Hooke(\Parameter) :  \StrainBasic( \ . \ ) \, d \Domain \right)^\frac{1}{2}
\end{equation}

\begin{equation}
\| \StressAlt \|_{\Hooke(\Parameter)^{-1}} = \left(  \int_\Domain \ . \  : \Hooke(\Parameter)^{-1}  : \ . \  \, \DVolume  \right)^\frac{1}{2}
\end{equation}


\subsection{Construction stress}

\begin{equation}
\forall \, \Parameter \in \ParameterSpace, \quad \StressFEM(\Parameter)
\approx
\StressHat(\Parameter) \Def   \StressFEMReducedHomo(\Parameter) +  \StressFEMLift(\Parameter)
\end{equation}


\begin{equation}
\forall \, \DispTest \in \SpaceDispFEMZero, \quad 
\int_\Domain \StressFEMReducedHomo(\Parameter) : \StrainTest \, \DVolume = 0 
\end{equation}


\begin{equation}
\NeumannBC(\Pos,\Parameter) = \sum_{i=1}^\NumberNeumannBCAffine \NeumannBCAffineI{i}(\Pos) \, \CoeffNeumannBCAffineI{i}(\Parameter) 
\end{equation}

\begin{equation}
\displaystyle
\forall \, i \in \llbracket 1, \, \NumberNeumannBCAffine   \rrbracket ,\, \forall \, \DispTest \in \SpaceDispFEMZero , 
 \quad
a(\FunctionAdStaticAffineI{i},\DispTest;\ParameterZero) = 
\int_\DDomainNeumann \NeumannBCAffineI{i} \cdot \DispTest \, \DSurface
\end{equation}

\begin{equation}
\StressFEMLift(\Parameter) \Def \sum_{i=1}^\NumberNeumannBCAffine \left( \Hooke(\ParameterZero) : \ \StrainBasic(\FunctionAdStaticAffineI{i}) \right) \CoeffNeumannBCAffineI{i}(\Parameter) 
\end{equation}


\begin{equation}
\SnapshotStressZero \Def  \{  \StressFEMHomo(\Parameter) \Def\StressFEM(\Parameter) - \StressFEMLift(\Parameter)  \, | \, \Parameter \in \ParameterSpaceDiscr  \}
\end{equation}


\begin{equation}
\forall \, \Parameter \in \ParameterSpace , \quad \StressReducedHat(\Parameter)   
= \sum_{i=1}^\NumberReducedBasisStress \ReducedBasisStressI{i} \, \ReducedCoeffStressI{i}(\Parameter)  +  \StressFEMLift(\Parameter)
\end{equation}

\begin{equation}
\begin{array}{l}
\displaystyle   (\ReducedBasisStressI{i})_{ i \in \llbracket 1,  \NumberReducedBasisStress \rrbracket } 
= \underset{
( \M{\widetilde{\phi}}_i^\star )_{ i \in \llbracket 1,  \NumberReducedBasis \rrbracket } , \, < \M{\widetilde{\phi}}_i^\star , \, \M{\widetilde{\phi}}_j^\star  >_{\Hooke(\ParameterZero)^{-1}} = \delta_{ij}
}{\text{argmin}} \quad  \widetilde{J} \left( (\M{\widetilde{\phi}}_i^\star )_{ i \in \llbracket 1,  \NumberReducedBasisStress \rrbracket } \right)
\\ \displaystyle
\widetilde{J} \left( ( \M{\widetilde{\phi}}_i^\star  )_{ i \in \llbracket 1,  \NumberReducedBasisStress \rrbracket } \right)
  =  \sum_{\Parameter \in \ParameterSpaceDiscr} 
  \left\| \StressFEMHomo(\Parameter) - \sum_{i=1}^\NumberReducedBasisStress \left< \StressFEMHomo(\Parameter) , \M{\widetilde{\phi}}_i^\star \right>_{\Hooke(\ParameterZero)^{-1}} \ \M{\widetilde{\phi}}_i^\star \right\|_{\Hooke(\ParameterZero)^{-1}}
\end{array}
\end{equation}

\begin{equation}
(\ReducedCoeffStressI{i})_{ i \in \llbracket 1,  \NumberReducedBasisStress \rrbracket } = \underset{   \Stress^\star(\Parameter) = 
\sum_{i=1}^\NumberReducedBasisStress \ReducedBasisStressI{i} \, \ReducedCoeffStressI{i}(\Parameter)  +  \StressFEMLift(\Parameter)
}{\text{argmin}} \left( \| \StressFEM(\Parameter)  - \Stress^\star(\Parameter)  \|_{\Hooke(\Parameter)^{-1}} \right)
\end{equation}


%\begin{equation}
 %\forall \, \StressTest \in \SpaceStressReducedZero,  \quad 
%\int_\Domain \StressFEMReducedHomo(\Parameter) : {\Hooke(\Parameter)^{-1}} :  \StressTest  \, \DVolume = 
%\int_\Domain  \StrainBasic \left(\DispFEMLift(\Parameter) \right) :  \StressTest  \, \DVolume 
%\end{equation}

\begin{equation}
\widetilde{\StiffnessFEM}^\text{r}(\Parameter) \, \widetilde{\ReducedCoeff}(\Parameter) = \widetilde{\ForceFEM}^\text{r}(\Parameter) 
%\StiffnessFEM^\text{r}(\Parameter) \, \ReducedCoeff(\Parameter) = \ForceFEM^\text{r}(\Parameter) + \ForceFEM^\text{r,p}(\Parameter)
\end{equation}


\subsection{lower bound}


\begin{equation}
\ErrorReducedApprox(\Parameter) \Def   \DispReducedEnhanced(\Parameter) - \DispReduced(\Parameter)
\end{equation}

\begin{equation}
\forall \,  \Parameter \in \ParameterSpace , \quad \LowerBound(\Parameter) \Def \frac{ \displaystyle
|  R( \ErrorReducedApprox(\Parameter) ; \Parameter)  |} 
{  \displaystyle
\|  \ErrorReducedApprox(\Parameter)  \|_{\Hooke(\Parameter)}
} 
\leq 
\| \ErrorReduced(\Parameter)  \|_{\Hooke(\Parameter)} 
\end{equation}

\subsection{adjoint}

\begin{equation}
\displaystyle  \text{Find} \ \V{z}^\text{h}(\Parameter) \in \mathcal{Z}^\text{h,0}(\Domain) \ \text{such that}  \ \forall \, \DispTest \in \mathcal{Z}^\text{h,0}(\Domain), 
 a(\DispTest, \V{z}^\text{h}(\Parameter) ;\Parameter) = \tilde{Q}(\DispTest)
\end{equation}

\begin{equation}
\displaystyle  \text{Find} \ \V{z}^\text{r}(\Parameter) \in \mathcal{Z}^\text{r,0}(\Domain) \ \text{such that}  \ \forall \, \DispTest \in \mathcal{Z}^\text{r,0}(\Domain),
\qquad
 a(\DispTest, \V{z}^\text{r}(\Parameter) ;\Parameter) = \tilde{Q}(\DispTest)
\end{equation}

\begin{equation}
\tilde{Q}(\ErrorReduced(\Parameter)) =  - R(\V{z}^\text{r} ; \Parameter) + a(\ErrorReduced(\Parameter), \V{z}^\text{h}(\Parameter)-\V{z}^\text{r}(\Parameter) ;\Parameter) 
%= R(\V{z}^\text{h}(\Parameter)-\V{z}^\text{r}(\Parameter) ;\Parameter)
\end{equation}

\begin{equation}
\tilde{Q}(\ErrorReduced(\Parameter)) =  a(\ErrorReduced(\Parameter), \V{z}^\text{h}(\Parameter)-\V{z}^\text{r}(\Parameter) ;\Parameter) \leq \| \ErrorReduced(\Parameter) \|_{\Hooke(\Parameter)} \, \| \V{z}^\text{h}(\Parameter)-\V{z}^\text{r}(\Parameter)  \|_{\Hooke(\Parameter)}
%= R(\V{z}^\text{h}(\Parameter)-\V{z}^\text{r}(\Parameter) ;\Parameter)
\end{equation}



\subsection{Resultats}

\begin{equation}
\forall \Parameter \in \ParameterSpace , \quad \DispFEM(\Parameter) = \bar{\Disp}(\Parameter) + \tilde{\Disp}^\text{h}(\Parameter) 
\end{equation}

\begin{equation}
\bar{\Disp}(\Parameter) = \StrainBasic^\text{M}(\Parameter) \, (\Pos - \bar{\Pos})
\end{equation}

\begin{equation}
\StrainBasic^\text{M}(\Parameter) =
\begin{pmatrix}
 \mu_2 & \mu_4 \\
 \mu_4 &  \mu_3
\end{pmatrix}
\end{equation}

\begin{equation}
\tilde{\Disp}(\Parameter)_{| \DDomain} = \V{0}
\end{equation}



\begin{equation}
\begin{array}{l} 
\displaystyle  \text{Find} \ \Tilde{\Disp}^\text{h}(\Parameter) \in \SpaceDispFEMZero\ \text{such that}  \ \forall \, \DispTest \in \SpaceDispFEMZero, 
\\ \displaystyle
\int_\Domain \StrainBasic(\Tilde{\Disp}^\text{h}(\Parameter)) : \Hooke(\Parameter) : \StrainBasic(\DispTest) \, \DVolume 
\\ \qquad \displaystyle = 
\int_\Domain \StrainBasic^\text{M}(\Parameter) : \Hooke(\Parameter) : \StrainBasic(\DispTest) \, \DVolume
\end{array} 
\end{equation}


\begin{equation}
\begin{array}{ll} 
\displaystyle   \tilde{\Output}(\Disp^\text{h}(\Parameter))  & \displaystyle  =  \M{\Sigma} :  \left( \frac{1}{|\Domain|} \int_\Domain \Hooke(\Parameter) : \StrainBasic(\Disp^\text{h}(\Parameter)) \, \DVolume \right)
\\ \displaystyle  
& \equiv \M{\Sigma} : \bar{\Hooke}(\Parameter) :  \StrainBasic^\text{M}(\Parameter)
\end{array} 
\end{equation}

\begin{equation}
 \left\{ \begin{array}{l} \displaystyle
\StrainBasic^\text{M} \equiv \frac{1}{2} \left( \V{e}_k \otimes \V{e}_l + \V{e}_l \otimes \V{e}_k \right)
\\ \displaystyle
 \M{\Sigma}  =\frac{1}{2} \left( \V{e}_i \otimes \V{e}_j + \V{e}_j \otimes \V{e}_i \right)
\end{array} \right.
\end{equation}

\begin{equation}
\tilde{\Output}(\Disp^\text{h}(\Parameter)) \equiv \bar{\Hooke}(\Parameter)_{ijkl}
\end{equation}

\begin{equation}
 \M{\Sigma} = \StrainBasic^\text{M}(\Parameter)
\end{equation}

\begin{equation}
\tilde{\Output}(\ErrorReduced(\Parameter))  = \int_ \Domain \StrainBasic(\ErrorReduced(\Parameter)): \Hooke(\Parameter) : \StrainBasic(\ErrorReduced(\Parameter)) \, \DVolume = \| \ErrorReduced(\Parameter)  \|_{\Hooke(\Parameter)}
\end{equation}

\begin{equation}
\Disp^\text{h}(\Parameter) 
\approx \sum_{i=1}^{\NumberReducedBasis} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter)  + \bar{\Disp}(\Parameter)  
\end{equation}

\begin{equation}
\DispReducedEnhanced(\Parameter) 
= \sum_{i=1}^{\NumberReducedBasisEnriched} \ReducedBasisI{i} \, \ReducedCoeffI{i}(\Parameter)  + \bar{\Disp}(\Parameter)  
\end{equation}

\begin{equation}
\StressHat(\Parameter)   
= \sum_{i=1}^\NumberReducedBasisStress \ReducedBasisStressI{i} \, \ReducedCoeffStressI{i}(\Parameter) \end{equation}

